Controlling for sparsity in sparse factor analysis models: adaptive latent feature sharing for piecewise linear dimensionality reduction

Ubiquitous linear Gaussian exploratory tools such as principle component analysis (PCA) and factor analysis (FA) remain widely used as tools for: exploratory analysis, pre-processing, data visualization and related tasks. However, due to their rigid assumptions including crowding of high dimensional data, they have been replaced in many settings by more flexible and still interpretable latent feature models. The Feature allocation is usually modelled using discrete latent variables assumed to follow either parametric Beta-Bernoulli distribution or Bayesian nonparametric prior. In this work we propose a simple and tractable parametric feature allocation model which can address key limitations of current latent feature decomposition techniques. The new framework allows for explicit control over the number of features used to express each point and enables a more flexible set of allocation distributions including feature allocations with different sparsity levels. This approach is used to derive a novel adaptive Factor analysis (aFA), as well as, an adaptive probabilistic principle component analysis (aPPCA) capable of flexible structure discovery and dimensionality reduction in a wide case of scenarios. We derive both standard Gibbs sampler, as well as, an expectation-maximization inference algorithms that converge orders of magnitude faster to a reasonable point estimate solution. The utility of the proposed aPPCA model is demonstrated for standard PCA tasks such as feature learning, data visualization and data whitening. We show that aPPCA and aFA can infer interpretable high level features both when applied on raw MNIST and when applied for interpreting autoencoder features. We also demonstrate an application of the aPPCA to more robust blind source separation for functional magnetic resonance imaging (fMRI).

==> Draft_text.tex <==


If we assume that each data point is associated with only a subset of latent variables (i.e. features), normally we can use binary variables to indicate these associations and denote our feature allocations.   


In this work we study a discrete latent variable approach to the feature allocation and subspace learning problem. Modelling 

Each data point
can be associated with a subset of the possible latent variables, which we refer to as the latent features of that data point.

 The binary variables in the
matrix indicate which latent feature is possessed by which data point, and
there is a potentially infinite array of features


In this work we propose novel feature allocation models using a naturally constrained urn model based on the hypergeometric distribution. This new framework allows for explicit control over the number of features used to express each point and enables a more flexible set of allocation distributions including feature allocations with different sparsity levels. PCA..FA
Motivated by the prohibitive slowness of ..we propose a scalable expectation-maximization inference algorithms which can converge orders of magnitude faster, significantly extending the utility of the proposed models. The proposed aFA outperforms previous FA models on data with varying levels of sparsity. We also demonstrate the proposed aPCA technique on hand written digits (MNIST) and fMRI data where it can be used for ...


can be used to capture a more flexible set of allocation distributions including different levels of sparseness. 

We ...FA and PCA

Each data point
can be associated with a subset of the possible latent variables, which we refer to as the latent features of that data point. The binary variables in the
matrix indicate which latent feature is possessed by which data point, and
there is a potentially infinite array of features


Learning however this feature allocation task, jointly with the feature subspaces is a long studied and difficult problem. Sparse analysis models and discrete continuous latent variables

Dicsrete-continious unifies a large set of approaches such as mixture of FA, single FA and sparse FA

We proposed/built a novel principal c
In this work we propose a fully Bayesian prior/model extension for data visualization and whitening based on orthogonality

Introducing sparseness

In this work we study some pitfalls of common latent feature linear models and propose novel 

...In this work we study novel latent feature models and propose some applications to classical techniques such as FA and PCA

A widely studied problem is subspace clustering

In this work we study how to construct novel/more efficient/better parametrized models...

Latent or hidden variables are an important component of many statistical models.
The role of these latent variables may be to represent properties of the objects or
data points being modelled that have not been directly observed, or to represent
hidden causes that explain the observed data


Many high-dimensional data, such as face images and motion sequences,
approximately lie in a union of low-dimensional subspaces. The corresponding subspace
clustering problem has been extensively studied in the literature to partition such highdimensional data into clusters corresponding to their underlying low-dimensional subspaces.
Low-dimensional intrinsic structures are often violated for real-world observations, as they
can be corrupted by errors or deviate from ideal models. We propose to address this by
learning a linear transformation on subspaces using nuclear norm as the modeling and optimization criteria.

Structure discovery in high dimensional data
Latent factor models are the canonical statistical tool for exploratory analyses of low-dimensional linear structure for a matrix of p features across n samples
Factor Analysis (FA) is a technique of fundamental importance that is widely used in classical and modern multivariate statistics, psychometrics, and econometrics. In this paper, we revisit the classical rank-constrained FA problem which seeks to approximate an observed covariance matrix (\BΣ) by the sum of a Positive Semidefinite (PSD) low-rank component (\BΘ) and a diagonal matrix (\BΦ) (with nonnegative entries) subject to \BΣ−\BΦ being PSD. 

We study latent feature models and propose some novel techniques for learning..
new models that address a and b
new inference that allows for scalable learnining

Latent feature learning 
Partial data visualization and subset whitening
Data visualization


Linear Gaussian
Latent feature approaches


We propose scalable Bayesian framework for augmentation of classical linear Gaussian techniques such a principal component analysis (PCA) and factor analysis (FA) models. First, a novel Bayesian nonparametric adaptive principal component analysis model is developed. Then we outline common issues with Bayesian nonparametric extensions to linear Gaussian techniques and propose a novel parametric discrete continuous latent variable framework based on the multivariate hypergeometric prior. Different inference mechanisms are studied and novel scalable expectation-maximization PCA and FA  aalgorithms are developed. We show that the adaptive PCA and adaptive FA methods can be successfully used in common applications for PCA and FA such as data visualization, dimensionality reduction and data whitening. A new avenue for discrete continuous graphical models is demonstrated, for accurate visualization of active brain regions during cognitive activities demonstrated using sample functional magnetic resonance imaging (fMRI) data.


In this work....adaptive Factor analysis and adaptive principal component analysis

In this work, we will directly extend the nonparametric FA model
of \citep{knowles2007infinite} to data visualization applications
by proposing a nonparametric PCA model with scalable inference.

We later show that while the nonparametric PPCA and FA models benefit
from additional flexibility, the underlying \textit{Indian buffet
process} (IBP) tends to create spurious latent factors and is inconsistent
for fixed concentration parameter (for formal proof of the latter
point, see \citet{Elvira2017}). This problem can be partially alleviated
via heuristic truncation of the least-represented factors, or using
an ensemble of multiple inference passes and identifying factors that
persist across multiple passes.


However, the \emph{multivariate hypergeometric prior }offers a more
principled solution via explicit control of the trade-off between
unique and shared factors. Furthermore, we show that the parameters
of the hypergeometric prior allow for control over the expected sharing,
while the IBP assumes log-linear growth of the number of factors \citep{di2020}
and decaying factor representation \citep{Teh2009indian}.

Independently, \cite{Elvira2017} also proposed a nonparametric extension
of PPCA using IBPs, but this used a different model on the projection
matrix $\mathbf{W}$ resulting in a very different inference algorithms.
Here, we present parametric and nonparametric variants of \emph{adaptive
}PPCA, as well as a generalization to flexible FA models. Using \textit{\emph{small
variance asymptotics}}, we show the explicit relationship between
adaptive PPCA models to classical PCA.





This model formulation is naturally understood in the context of data visualization. 

to grow the number of features used to represent the full training dataset, without inferring  

....specifies the maximum feature capacity.., but the features available to each element are limitted and unknown

the multivariate hypergeometric distribution as a model for feature allocation

Where ###  
based on latent class \citep{tipping1999mixtures,archambeau2008mixtures,ghahramani1996algorithm} or latent feature linear Gaussian models (references). The latent feature methods we study here explicitly model more flexible cluster topology which accounts for overlapping clusters and mixed group membership. Parametric feature allocation methods assume a fixed number of features which have independent allocation probability. Nonparametric factor analyzers assume 
In this work we 
Feature allocation is normally governed by a Beta-Bernoulli distribution or a nonparametric extension of such. In exploratory analysis the Beta parameters are shared across all features or a concentration parameter governs the nonparametric Beta process. In either case ,,,///

The challenge is 
However, feature sharing is typically being modelling using  conjugate Beta-Bernoulli distribution pair or Beta process..

This is normally done by replacing the Dirichlet-Multinomial conjugate pair as a modelling choice with a independent Beta-Bernoulli 

Previous latent feature Gaussian models adopt Beta 

This way this achieved is by placing a Beta-Bernoulli prior over discrete latent variables. Paramatric Beta-Bernoulli can in principle....but
The more flexible latent feature models such as the Bayesian nonparametric factor analysis or the nonparametric independent component analysis replace the Beta-Bernoulli with infinite capacity Beta process prior. However, the Beta process fixed..sublinear feature popularity. The Beta process is parametrised by a single concentration parameter and is inconsistent. This forces..rigit assumtions about the feature sharing. Here we propose an alternative, 


The problem is that latent feature models are based on Beta 
Latent feature models when introduced, what for...Latent feature models for data visualization
The latent feature models models use Beta-Bernoulli distribution or Beta process in the nonparametric setup, to model the distribution over the latent features. This problem 
Latent feature models based on the Beta-Bernoulli distribution, the IBP or the Beta process, do not allow for flexible control over the latent space. Typically, they enforce  



which has motivated development of flexible \textit{latent
feature} models such as nonparametric factor analysis \citep{knowles2007infinite,Paisley2009,rai2009infinite}.
Latent feature models are useful for modeling more complex topological
groupings in the data, accounting for overlaps and mixed group membership
data. In this work, we will directly extend the nonparametric FA model
of \citep{knowles2007infinite} to data visualization applications
by proposing a nonparametric PCA model with scalable inference.

We later show that while the nonparametric PPCA and FA models benefit
from additional flexibility, the underlying \textit{Indian buffet
process} (IBP) tends to create spurious latent factors and is inconsistent
for fixed concentration parameter (for formal proof of the latter
point, see \citet{Elvira2017}). This problem can be partially alleviated
via heuristic truncation of the least-represented factors, or using
an ensemble of multiple inference passes and identifying factors that
persist across multiple passes.


However, the \emph{multivariate hypergeometric prior }offers a more
principled solution via explicit control of the trade-off between
unique and shared factors. Furthermore, we show that the parameters
of the hypergeometric prior allow for control over the expected sharing,
while the IBP assumes log-linear growth of the number of factors \citep{di2020}
and decaying factor representation \citep{Teh2009indian}.

Independently, \cite{Elvira2017} also proposed a nonparametric extension
of PPCA using IBPs, but this used a different model on the projection
matrix $\mathbf{W}$ resulting in a very different inference algorithms.
Here, we present parametric and nonparametric variants of \emph{adaptive
}PPCA, as well as a generalization to flexible FA models. Using \textit{\emph{small
variance asymptotics}}, we show the explicit relationship between
adaptive PPCA models to classical PCA.










In this work, we will directly extend the nonparametric FA model
of \citep{knowles2007infinite} to data visualization applications
by proposing a nonparametric PCA model with scalable inference.



However, the assumption that data lies
in distinct non-overlapping clusters of linear subspaces is quite
restrictive, which has motivated development of flexible \textit{latent
feature} models such as nonparametric factor analysis \citep{knowles2007infinite,Paisley2009,rai2009infinite}.


These models are commonly used for subspace clustering and restrictively assume fixed  

These techniques...subspace clustering...(Bayesian hierarchical mixture of factor analyzers reference)

(http://mlg.eng.cam.ac.uk/zoubin/papers/nips99.pdf Variational inference mixture of factor analysis)
Explicitly modelling potential partitions and latent memberships...has motivated work on hierarchical models such as...

Subspace clustering
From the perspective of directly discovering non-overlapping
subspaces of data (i.e.\textit{ subspace clustering}), extensions
based on mixtures of PPCA models and FA models have been proposed
\citep{tipping1999mixtures,archambeau2008mixtures,ghahramani1996algorithm}.
These were later extended to create more flexible models which can
also infer the optimal dimensionality of cluster subspaces, as well
as the number of separate mixture components supported by the data
\citep{Chen2010,Wang2015}. 

However, the assumption that data lies
in distinct non-overlapping clusters of linear subspaces is quite
restrictive, which has motivated development of flexible \textit{latent
feature} models such as nonparametric factor analysis \citep{knowles2007infinite,Paisley2009,rai2009infinite}.
Latent feature models are useful for modeling more complex topological
groupings in the data, accounting for overlaps and mixed group membership
data. In this work, we will directly extend the nonparametric FA model
of \citep{knowles2007infinite} to data visualization applications
by proposing a nonparametric PCA model with scalable inference.


This work however ...does not allow for Bayesian treatment over ...

Posing the problem as discrete continuous

Latent feature models are useful for modeling more complex topological
groupings in the data, accounting for overlaps and mixed group membership
data. In this work, we will directly extend the nonparametric FA model
of \citep{knowles2007infinite} to data visualization applications
by proposing a nonparametric PCA model with scalable inference.

This is where latent feature 

PCA suffers from the fact that each principal component is a linear
combination of all the original variables, thus it is often difficult to interpret the results. We
introduce a new method called sparse principal component analysis (SPCA) using the lasso
(elastic net) to produce modified principal components with sparse loadings

A challenge that all of these linear Gaussian techniques share (also
common for flexible nonlinear continuous latent variable models, i.e.
see \citet{dai2015spike}) is that we assume matrix $\mathbf{W}$
is applied across all data points. This assumption typically enables
simpler training via matrix algebra, instead of iterative inference
methods.
###############
Sparse principal component analysis methods
####
Sparse factor analysis methods
#####
PPCA extensions have been introduced that offer robustness to outliers
and data corruption \citep{SchmittFastHCS}, but challenges caused
by multi-modalities in high dimensional data require formal model
augmentation. From the perspective of directly discovering non-overlapping
subspaces of data (i.e.\textit{ subspace clustering}), extensions
based on mixtures of PPCA models and FA models have been proposed
\citep{tipping1999mixtures,archambeau2008mixtures,ghahramani1996algorithm}.
These were later extended to create more flexible models which can
also infer the optimal dimensionality of cluster subspaces, as well
as the number of separate mixture components supported by the data
\citep{Chen2010,Wang2015}. However, the assumption that data lies
in distinct non-overlapping clusters of linear subspaces is quite
restrictive, 







There are many Bayesian nonparametric extensions of the linear Gaussian
model \eqref{eq:Linear-Gaussian-2}. \citet{knowles2007infinite}
introduced \emph{infinite sparse factor analysis }(isFA) by including
a binary indicator variable \textbf{$\mathbf{z}$} within the latent
space, and by placing the IBP \citep{Ghahramani2006} prior (see section
\ref{subsec:IBP}) on \textbf{$\mathbf{z}$,} isFA is able to learn
an infinite number of hidden sources (where only a finite number
of sources are non-zero); \citet{Paisley2009} replace the IBP prior
with a Beta process\footnote{The IBP is the marginal process of the beta-Bernoulli process \citep{thibaux2007hierarchical}}
\cite{hjort1990nonparametric} to derive the \emph{Beta process factor
analysis model}; this allows for faster \textit{variational} inference when compared to the Gibbs used by \citet{knowles2007infinite}.
By placing a Laplacian prior on $\mathbf{x}$, \citet{knowles2007infinite}
obtained a version of infinite independent components analysis (iICA).


for most visualization applications
we set $L=2$ or $L=3$. 





Here we will propose a different model for the matrix $\mathbf{Z}$
which allows for explicit control over the number of latent subspaces
$L$ used to decompose each observation to a lower dimensional space.
Note that $L$ plays a very different role to $K$: it is as most
$K$, but more often is much less than $K$, ; here $K$ denotes the
number of unique orthogonal linear subspaces which we will use to
reduce the original data $\mathbb{R}^{D}$ into the lower dimensional,
latent space; each input data point can be associated with different
subset of $L$ subspaces, selected from a total of $K$ subspaces.
So, any single point is actually represented by lower dimensional
spaces subsets of $\mathbb{R}^{L}$. In the case of PPCA models the
orthogonality assumption $\boldsymbol{\mathrm{w}}_{i}\perp\boldsymbol{\mathrm{w}}_{j}\;\forall i\neq j$
for the columns of $\mathbf{W}$ implies that $K\leq D$, but if
we wish to apply the same alternative prior to $\mathbf{Z}$ in augmented
FA or ICA models \citep{Paisley2009,knowles2007infinite}, $K$ would
need to be arbitrarily large. Put another way, $K$ accounts for the
global sharing of structure across overlapping groups of data points
with common features; if $K$ is large enough, each point can, in
principle, be associated with its own number of $L$, unique subspaces
and which coincides with subspace clustering. But, as $K$ reduces,
more of these subspaces are constrained to be shared across regions
of the data space. Therefore, $L$ acts much like the number of latent
dimensions in traditional linear dimensionality reduction techniques,
but here $L$ is constrained by $K$. This allows us to interpret
$L$ as the \emph{local capacity }of the model and $K$ controls \emph{global
}capacity or sharing. If $L=K$ we recover classical latent factor
models, since all features are associated with all observed data
points. As $K-L$ increases, more local structure of the manifold
can be captured; where the number of total subspaces is $\tbinom{K}{L}$.

To implement this model, we place a \textit{multivariate hypergeometric
distribution} \citep{chesson1976non} as a prior over all the latent
feature indicators $\mathbf{Z}$:



\begin{equation}
\mathrm{P}\left(\mathbf{Z}\vert K,L,m_{1,\ldots,K}=1\right)=\prod_{n=1}^{N}\frac{\binom{1}{z_{1,n}}\binom{1}{z_{2,n}}\times\ldots\times\binom{1}{z_{K,n}}}{\binom{K}{L}}\label{eq:Zprior-1-1}
\end{equation}
for given values of $L$ and $K$. For \eqref{eq:Zprior-1-1} $z_{k,n}\in\left\{ 0,1\right\} $
and we have $\sum_{k=1}^{K}z_{k,n}=L$; for most visualization applications
we set $L=2$ or $L=3$. This ability to isolate sufficiently detailed
structure from the global input space comes at the cost of not having
the \emph{re-enforcement effect }of Bayesian nonparametrics; this
is because the multivariate hypergeometric prior acts as an uninformative
prior under the explicitly constrained dimensionality.








The factor analysis models...we do new one...also we make it fast

Next, we show that we can also relax the orthogonality constraint
on the columns of the matrix $\mathbf{W}$ of parametric aPPCA, to
obtain a flexible \textit{adaptive factor analysis} (aFA) model.
We propose a scalable expectation-maximization (EM) algorithm in which
we directly optimize $\mathbf{W}$, marginalize the latent $\mathbf{X}$
and infer the MAP estimate for the latent $\mathbf{Z}$. We will show
that the algorithm is a more scalable and naturally truncated version
of isFA \citep{knowles2007infinite} suited to different sparsity
levels of $\mathbf{Z}$.

